LightLayers: Parameter Efficient Dense and Convolutional Layers for Image Classification

Deep Neural Networks (DNNs) have become the de-facto standard in computer vision, as well as in many other pattern recognition tasks. A key drawback of DNNs is that the training phase can be very computationally expensive. Organizations or individuals that cannot afford purchasing state-of-the-art hardware or tapping into cloud-hosted infrastructures may face a long waiting time before the training completes or might not be able to train a model at all. Investigating novel ways to reduce the training time could be a potential solution to alleviate this drawback, and thus enabling more rapid development of new algorithms and models. In this paper, we propose LightLayers, a method for reducing the number of trainable parameters in deep neural networks (DNN). The proposed LightLayers consists of LightDense andLightConv2D layer that are as efficient as regular Conv2D and Dense layers, but uses less parameters. We resort to Matrix Factorization to reduce the complexity of the DNN models resulting into lightweight DNNmodels that require less computational power, without much loss in the accuracy. We have tested LightLayers on MNIST, Fashion MNIST, CI-FAR 10, and CIFAR 100 datasets. Promising results are obtained for MNIST, Fashion MNIST, CIFAR-10 datasets whereas CIFAR 100 shows acceptable performance by using fewer parameters.

==> takeouts.tex <==
% 
%We aim to develop an accurate and robust method for surgical instrument segmentation from endoscopic images based on computer vision techniques. However, one of the significant problem in the field is lack of publicly available dataset for benchmarking the algorithms and improving the benchmark on the same datasets\cite{jha2020kvasir}. For the Kvasir-instrument dataset, we have used UNet architecture, which is common semantic segmentation based architecture for medical image segmentation tasks. Next, we provide a baseline algorithm that provides and invite multimedia researcher to improve the baseline methods. In this paper, we present our approach for binary instrument segmentation on the endoscopic instrument segmentation dataset. 
